Updated Status of the Global Electroweak Fit and Constraints on New Physics

We present an update of the Standard Model fit to electroweak precision data. We include newest experimental results on the top quark mass, the W mass and width, and the Higgs boson mass bounds from LEP, Tevatron and the LHC. We also include a new determination of the electromagnetic coupling strength at the Z pole. We find for the Higgs boson mass (91 +30 -23) GeV and (120 +12 -5) GeV when not including and including the direct Higgs searches, respectively. From the latter fit we indirectly determine the W mass to be (80.360 +0.014 -0.013) GeV. We exploit the data to determine experimental constraints on the oblique vacuum polarisation parameters, and confront these with predictions from the Standard Model (SM) and selected SM extensions. By fitting the oblique parameters to the electroweak data we derive allowed regions in the BSM parameter spaces. We revisit and consistently update these constraints for a fourth fourth fermion generation, two Higgs doublet, inert Higgs and littlest Higgs models, models with large, universal or warped extra dimensions and technicolour. In most of the models studied a heavy Higgs boson can be made compatible with the electroweak precision data.

==> Figures_Para/FullFitTable.tex <==
\begin{table}
\setlength{\tabcolsep}{0.0pc}
{\small
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccccc} 
\hline\noalign{\smallskip}
& & Free & \multic{2}{c}{Results from global EW fits:} & \multic{1}{c}{\em Complete fit w/o}   \\[-0.1cm]
\rs{Parameter} & \rs{Input value} & in fit & \multic{1}{c}{\em Standard fit} & \multic{1}{c}{\em Complete fit} & \multic{1}{c}{\em exp. input in line} \\
%
\noalign{\smallskip}\hline\noalign{\smallskip}
$M_{Z}$ {\ft [GeV]} &  $91.1875\pm0.0021$ & yes &  $91.1874\pm0.0021$ &  $91.1877\pm0.0021$ &  $91.1941^{\,+0.0151}_{\,-0.0143}$\\
$\Gamma_{Z}$ {\ft [GeV]} &  $2.4952\pm0.0023$ & -- &  $2.4959\pm0.0015$ &  $2.4955\pm0.0014$ &  $2.4953\pm0.0016$\\
$\sigma_{\rm had}^{0}$ {\ft [nb]} &  $41.540\pm0.037$ & -- &  $41.478\pm0.014$ &  $41.478\pm0.014$ &  $41.469\pm0.015$\\
$R^{0}_{\l}$ &  $20.767\pm0.025$ & -- &  $20.770\pm19.770$ &  $20.741^{\,+0.018}_{\,-0.017}$ &  $20.718\pm0.026$\\
$A_{\rm FB}^{0,\l}$ &  $0.0171\pm0.0010$ & -- &  $0.01641\pm0.0002$ &  $0.01625^{\,+0.0002}_{\,-0.0001}$ &  $0.01625^{\,+0.0002}_{\,-0.0001}$\\
 $A_\ell$ $^{(\star)}$  & $0.1499\pm0.0018$ & --  & $0.1479\pm0.0010$ & $0.1472^{+0.0010}_{-0.0005}$ & --\\
$A_{c}$ &  $0.670\pm0.027$ & -- &  $0.6683^{\,+0.00044}_{\,-0.00043}$ &  $0.6680^{\,+0.00043}_{\,-0.00025}$ &  $0.6680^{\,+0.00043}_{\,-0.00024}$\\
$A_{b}$ &  $0.923\pm0.020$ & -- &  $0.93469^{\,+0.00009}_{\,-0.00008}$ &  $0.93464^{\,+0.00007}_{\,-0.00005}$ &  $0.93465\pm0.00005$\\
$A_{\rm FB}^{0,c}$ &  $0.0707\pm0.0035$ & -- &  $0.0741\pm0.0005$ &  $0.0738^{\,+0.0005}_{\,-0.0003}$ &  $0.0738^{\,+0.0005}_{\,-0.0003}$\\
$A_{\rm FB}^{0,b}$ &  $0.0992\pm0.0016$ & -- &  $0.1037\pm0.0007$ &  $0.1032^{\,+0.0007}_{\,-0.0004}$ &  $0.1038^{\,+0.0003}_{\,-0.0005}$\\
$R^{0}_{c}$ &  $0.1721\pm0.0030$ & -- &  $0.17229^{\,+0.00007}_{\,-0.00006}$ &  $0.17229^{\,+0.00007}_{\,-0.00006}$ &  $0.17229\pm0.00006$\\
$R^{0}_{b}$ &  $0.21629\pm0.00066$ & -- &  $0.21575^{\,+0.00005}_{\,-0.00008}$ &  $0.21574^{\,+0.00005}_{\,-0.00008}$ &  $0.21575\pm0.00001$\\
$\sinleff(Q_{\rm FB})$ &  $0.2324\pm0.0012$ & -- &  $0.23141^{\,+0.00012}_{\,-0.00013}$ &  $0.23149^{\,+0.00007}_{\,-0.00012}$ &  $0.23149^{\,+0.00008}_{\,-0.00012}$\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$M_{H}$ {\ft [GeV]} $^{(\circ)}$ & Likelihood ratios & yes & $94^{+ 30[+ 74]}_{- 24[- 43]}$ & $120^{+ 12[+ 23]}_{-  5[-  6]}$ & $94^{+ 30[+ 74]}_{- 24[- 43]}$\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$M_{W}$ {\ft [GeV]} &  $80.399\pm0.023$ & -- &  $80.382^{\,+0.014}_{\,-0.015}$ &  $80.371^{\,+0.007}_{\,-0.010}$ &  $80.358^{\,+0.017}_{\,-0.010}$\\
$\Gamma_{W}$ {\ft [GeV]} &  $2.085\pm0.042$ & -- &  $2.093\pm0.001$ &  $2.092\pm0.001$ &  $2.091^{\,+0.002}_{\,-0.001}$\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$\mc$ {\ft [GeV]} &  $1.27^{\,+0.07}_{\,-0.11}$ & yes &  $1.27^{\,+0.07}_{\,-0.11}$ &  $1.27^{\,+0.07}_{\,-0.11}$ & -- \\
$\mb$ {\ft [GeV]} &  $4.20^{\,+0.17}_{\,-0.07}$ & yes &  $4.20^{\,+0.16}_{\,-0.07}$ &  $4.20^{\,+0.16}_{\,-0.07}$ & -- \\
$m_{t}$ {\ft [GeV]} &  $173.3\pm1.1$ & yes &  $173.4\pm1.1$ &  $173.7\pm1.0$ &  $176.8\pm3.3$$^{(\bigtriangledown)}$\\
$\dalphaHadMZ$ $^{(\dag\bigtriangleup)}$ &  $2749\pm  10$ & yes & $2750\pm  10$ & $2748\pm  10$ & $2729^{+  57}_{-  50}$\\
$\alpha_{s}(M_{Z}^{2})$ & -- & yes &  $0.1193\pm0.0028$ &  $0.1194\pm0.0028$ &  $0.1194\pm0.0028$\\
\noalign{\smallskip}\hline\noalign{\smallskip}
$\deltatheo M_W$ {\ft [MeV]}  & $[-4,4]_{\rm theo}$ & yes  & $4$ & $4$ & -- \\
$\deltatheo \sinleff$ $^{(\dag)}$  & $[-4.7,4.7]_{\rm theo}$ & yes  & $4.7$ & $4.7$ & -- \\
\noalign{\smallskip}\hline
\noalign{\smallskip}
\end{tabular*}
{\ft
$^{(\star)}$Average of LEP ($A_\ell=0.1465\pm0.0033$) and SLD ($A_\ell=0.1513\pm0.0021$) measurements.
The {\em complete fit} w/o the LEP (SLD) measurement gives $A_\ell=$ $0.1473^{\,+0.0010}_{\,-0.0006}$ 
($A_\ell=$ $0.1469^{\,+0.0007}_{\,-0.0005}$ 
).
$^{(\circ)}$In brackets the $2\sigma$. 
$^{(\dag)}$In units of $10^{-5}$.
$^{(\bigtriangleup)}$Rescaled due to $\alpha_s$ dependency.
$^{(\bigtriangledown)}$Ignoring a second less significant minimum, \cf Fig.~\ref{fig:topscan} and Eq.~(\ref{eq:mtop_completefit}).
}}
\label{tab:results}
\end{table}

